Cooperative Object Transportation using Gibbs Random Fields

This paper presents a novel methodology that allows a swarm of robots to perform a cooperative transportation task. Our approach consists of modeling the swarm as a {\em Gibbs Random Field} (GRF), taking advantage of this framework's locality properties. By setting appropriate potential functions, robots can dynamically navigate, form groups, and perform cooperative transportation in a completely decentralized fashion. Moreover, these behaviors emerge from the local interactions without the need for explicit communication or coordination. To evaluate our methodology, we perform a series of simulations and proof-of-concept experiments in different scenarios. Our results show that the method is scalable, adaptable, and robust to failures and changes in the environment.

==> sections/algorithm.tex <==
\begin{algorithm}[t]
\caption{Calculate robot $i$ velocity at time $t+1$}\label{alg:metropolis}
\Procedure{Update}{$\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)}$} 
 \State $\mathbf{V}^{(0)} \gets \mathbf{v_i}^{(t)}$, \Comment{Set of velocities} 
 \State $\mathbf{U}^{(0)} \gets H(\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)})$, \Comment{Set of potential energies} 
 \For{$k \gets 1$ to $\mathcal{I}$}
%  \State $\mathbf{v}_{prev} \gets \mathbf{V}$(end),  \Comment{Get the last element of $\mathbf{V}$} 
%  \State $\mathbf{u}_{prev} \gets \mathbf{U}$(end),  \Comment{Get the last element of $\mathbf{U}$} 
 \State $\bar{\mathbf{v}} \gets N(\mathbf{v_i}^{(t)}, \mathbf{\Sigma})$,    \Comment{Gaussian sampling} 
 \State $\bar{\mathbf{u}} \gets  H(\mathbf{q_i}^{(t)}, \bar{\mathbf{v}})$,
 \State $\Delta E \gets \bar{\mathbf{u}} - \mathbf{U}^{(k-1)}$,      \Comment{Potential energy variation}
 \State $g \gets exp(-\Delta E)$,   \Comment{Compute the gibbs energy}
 \State $r \gets \mathcal{U}(0, 1)$,   \Comment{Uniform sampling}
 \If{$(\Delta E < 0) \lor (r < g)$ } \Comment{Sample is accepted}
    \State $\mathbf{V}^{(k)} \gets \bar{\mathbf{v}}$,
    \State $\mathbf{U}^{(k)} \gets \bar{\mathbf{u}}$,
    \Else \Comment{Sample is rejected}
    \State $\mathbf{V}^{(k)} \gets  {\mathbf{V}^{(k-1)}}$,
    \State $\mathbf{U}^{(k)} \gets  {\mathbf{U}^{(k-1)}}$,
    \EndIf
 \EndFor
%  \State $\mathbf{V} \gets \mathbf{V}^{(j,...,\mathcal{I})}$, \Comment{Reject the first j velocities}
 \State $\mathbf{v_i}^{(t+1)} \gets  (\mathbf{V}^q + ...+\mathbf{V}^\mathcal{I})/(\mathcal{I}-q)$, \Comment{Average velocity}
 \State \textbf{return} $\mathbf{v_i}^{(t+1)}$
\EndProcedure
\end{algorithm}

==> sections/temp/03_background.tex <==
% \section{Background}
% \label{sec:background}
% In this section, we overview some concepts about \textit{Gibbs Random Fields} (GRFs) explaining their properties and why they make sense in a swarm robotics context.
% A GRF is a probabilistic graphical model that is a particular case of the  \textit{Markov Random Field} (MRF) when the joint probability density of the random variables is strictly positive. GRF models are based on local interactions between neighboring agents. The Markov property is a conditional property that allows one to ignore more distant information as soon as local information is provided. The Hammersley-Clifford theorem establishes the equivalence between a MRF and a GRF~\cite{kindermann1980markov}. %Here we are not going to demonstrate such equivalence, but only present an overview of a MRF towards a GRF.

% To describe these models succinctly, assume an undirected graph $\mathbf{G} = (\mathbf{V},\mathbf{E})$ with vertices as spatial sites and indexed by $v = 1, 2, . . . , \eta$. A random field on $\mathbf{G}$ is as collection of random variables $\mathbf{X} = \{X_{v}\}_{v \in \mathbf{V}}$ and, for each $v \in \mathbf{V}$, let $\Lambda_v$ be finite set called the phase space for site $v$ that represents where the random variable $X_v$ takes it values.
% % ≜ -> is equal by definition to  
% An instance of $\mathbf{X}$ establishes a state of the random field $x = \{(x_1,..., x_\eta): x_v \in \Lambda_v, v \in \mathbf{V}\}$ and the product space $\Lambda \triangleq \Lambda_1 \times ... \times \Lambda_\mathbf{\eta} $ forms the configuration space. 

% A neighborhood system on $\mathbf{V}$ is a family $\mathcal{N} = \{\mathcal{N}_v\}_{v \in \mathbf{V}}$, where $\mathcal{N}_v \subset \mathbf{V}$ is the set of neighbors for site $v$ satisfying $v/\mathcal{N}_v$ and $r \in \mathcal{N}_v \Leftrightarrow v \in \mathcal{N}_r$. 
% %
% The neighborhood system induces the configuration of the undirected graph $\mathbf{G}$ by setting 
% %with vertices $v, r \in \mathbf{V}$, and 
% an edge $\{v,r\} \in \mathbf{E}$ between $v$ and $r$ if and only if $r \in \mathcal{N}_v$. A set $\mathcal{C} \subset \mathbf{V}$ is called a \textit{clique} if all elements of $\mathcal{C}$ are neighbors of each other. 

% Thus, a random field $\mathbf{X}$ is called an MRF concerning the neighborhood system $\mathcal{N}$ if, $\forall v \in \mathbf{V}$,
% \begin{equation}
% \displaystyle{
%     P(X_v=x_v \text{$|$} (X_r=x_r)_{r \neq v}) = P (X_v=x_v \text{$|$} (X_r=x_r)_{r \in \mathcal{N}_v})},
% \label{eq:mrf}
% \end{equation}
% %where $\displaystyle{P(\cdot|\cdot)}$ denotes the conditional probability of the event $e_1$ given that the event $e_2$ happens. 
% which indicates that the probability of the site $v$ assuming the state $x_v$ given the state of all other sites is equal to the probability of $v$ assuming the same state $x_v$ given only the states of neighboring sites. Such a definition reflects the local characteristics of the MRF constrained by the local Markov properties~\cite{koller2009probabilistic} and is convenient to model robotics swarms, since it implies the conditional independence of information coming from outside a neighborhood system, which supports the requirement of local interactions. 

% %A remark for (\ref{eq:mrf}) is that it reflects the local characteristics of the MRF constrained by the local Markov properties~\cite{koller2009probabilistic}. Such constraints may be convenient to model swarm robots since it implies the independence of information coming from outside a neighborhood system, which supports the requirement of local interaction. 

% % By definition, an MRF satisfies the following Markov properties:  
% %  \subsubsection{Pairwise Markov property} Any two non-neighbors variables are conditionally independent given all other variables: 
% %  \begin{align*}
% %      X_{u} \perp \!\!\!\perp X_{v} \mid X_{V \setminus \{u,v\}}.
% %  \end{align*}

% % \subsubsection{Local Markov property} A variable is conditionally independent of all other variables given its neighbors:
% % \begin{align*}
% %  X_{v}\perp \!\!\!\perp X_{V\setminus \mathcal{N}_{v+}}\mid X_{\mathcal{N}_v},
% %  \end{align*}
% % where $\mathcal{N}_v$ is the set of neighbors of $v$, and $\mathcal{N}_{v+}=v\cup \mathcal{N}_v$ is the closed neighborhood of $v$.

% % \subsubsection{Global Markov property} Any two subsets of variables are conditionally independent given a separating subset:
% %     \begin{align*}
% %     X_{A}\perp \!\!\!\perp X_{B}\mid X_{S},
% %     \end{align*}
% % where a separating subset $S$ is one in which every path from a subset $A$ to a subset $B$ passes through it.
% %
% % In general, the last property is stronger than the second one, which in turn is stronger than the first one. But, if the probability is positive, the above three Markov properties are equivalent~\cite{koller2009probabilistic}. 
% %Such constraints may be convenient to model swarm robots since it implies the independence of information coming from outside a neighborhood system, which supports the requirement of local interaction. 

% A GRF is a particular application for (\ref{eq:mrf}) when its joint probability density can be represented by the Gibbs measure. A Gibbs measure is a generalization of the canonical ensemble to infinite systems, which gives the probability of the system $\mathbf{X}$ being in the state $x$. Formally, let us denote a potential $\mathbf{U}$ as a family $\displaystyle{\{U_A : A \subset \mathbf{V}\}}$ of functions on the configuration space $\Lambda$, where $U_A : \Lambda \rightarrow \mathbb{R}$, and $U_A(x)$ depends only on $x_A \triangleq \{x_v: v \in A\}$. At the end, $U_A$ is only a function of the values at the sites contained in the set $A$, that is $\displaystyle{U_A(x) \equiv U_A(x_A)}$. In this way, given a potential $\mathbf{U}$, the potential energy $H(x)$ for configuration $x$ is defined as
% \begin{equation}
% H(x) = \sum \limits_{A \subset \mathbf{V}} U_A(x_A).
% \label{eq:potentialenergy1}
% \end{equation}

% By definition~\cite{kindermann1980markov}, if $U_A \equiv 0$ whenever $A$ is not a \textit{clique} or a singleton, $\mathbf{U}$ is called a nearest-neighbor potential. If $U_A \equiv 0$ whenever $A$ is not a pair or a singleton, $\mathbf{U}$ is called a pairwise potential. $\mathbf{U}$ is called a pairwise, nearest-neighbor potential if it is both a pairwise potential and a nearest-neighbor potential. In particular, for a pairwise, nearest-neighbor potential $U$, we can write (\ref{eq:potentialenergy1}) as
% \begin{equation}
% H(x) = \sum \limits_{v \in \mathbf{V}} U_{\{v\}}(x_v) + \sum \limits_{(v,t) \in \mathbf{V}  \times \mathbf{V}, t \in \mathcal{N}_v} U_{\{v,t\}}(x_v, x_t).
% \label{eq:potentialenergy2}
% \end{equation}

% Finally, a random field $\mathbf{X}$ is called a GRF if,
% \begin{equation}
%     P(\mathbf{X} = x) = \frac{1}{Z}e^{-\frac{H(x)}{T}}, \textrm{ with } Z = \sum \limits_{z} e^{-\frac{H(x)}{T}},
%     \label{eq:gibbsdistribution}
% \end{equation}
% where $Z$ is the partition function (normalizing constant); $T$ is interpreted as temperature in the context of statistical physics; and $\frac{1}{Z}e^{-\frac{H(x)}{T}}$ is called Gibbs distribution. 
% %A remark for (\ref{eq:gibbsdistribution}) is that a higher-energy state implies a lower probability and that the influence of energy on probability increases as $T$ decreases. 

% Researchers in statistical mechanics and mathematics usually applied the GRF to describe the distribution of system configurations at the thermodynamic equilibrium or to measure the probability of such a system to yield the desired state. One of the challenges of directly evaluating~(\ref{eq:gibbsdistribution}) is the high cardinality of the configuration space, which makes the computation of $Z$ intractable.

% A typical approach to sequential sampling states in a configuration space given a probability function consists of using Markov Chain Monte Carlo (MCMC) methods, such as the Metropolis algorithm~\cite{hastings1970monte}. A process to parallely sample over~(\ref{eq:gibbsdistribution}) is described in the next section.







==> sections/temp/04_methodology_2.tex <==

\section{Methodology}
\label{sec:methodology}
In this section, we briefly overview some concepts about \textit{Gibbs Random Fields} (GRFs)\footnote{See Rezeck et al.\cite{} for more details}  and extend it concepts to the context of swarm robotics and present our modeling and control strategy to coordinated a swarm of robots to cohesive navigate through a environment and cooperatively transport an object toward its goal location.

The general idea of our methodology consists of modeling the configuration of a swarm of robots as a GRF and then sampling velocities for each robot in a decentralized way, which leads the entire swarm to a convergence towards the global minimum of the potential.

\subsection{Background} 
\label{subsec:background}
A GRF is a probabilistic graphical model that is a particular case of the  \textit{Markov Random Field} (MRF) when the joint probability density of the random variables is strictly positive. GRF models are based on local interactions between neighboring agents. The Markov property is a conditional property that allows one to ignore more distant information as soon as local information is provided. The Hammersley-Clifford theorem establishes the equivalence between a MRF and a GRF~\cite{kindermann1980markov}. %Here we are not going to demonstrate such equivalence, but only present an overview of a MRF towards a GRF.

To describe these models succinctly, assume an undirected graph with vertices indexed as spatial sites. A random field on the graph consist of a collection of random variables, associated with its respective vertices, and represent the probability of that vertex assuming a certain state. A neighborhood system consist of a set of neighbors for each vertex and satisfies symmetry and non-self-inclusion. The neighborhood system induces the configuration of the undirected graph by setting an edge between two vertices if they are neighbors.

Thus, a random field on the graph is called an MRF concerning the neighborhood system if, for each vertex, this statement is true,
\begin{equation}
\displaystyle{
    P(X_v=x_v \text{$|$} (X_r=x_r)_{r \neq v}) = P (X_v=x_v \text{$|$} (X_r=x_r)_{r \in \mathcal{N}_v})},
\label{eq:mrf}
\end{equation}
and indicates that the probability of the site $v$ assuming the state $x_v$ given the state of all other sites is equal to the probability of $v$ assuming the same state $x_v$ given only the states of neighboring sites. Such a definition reflects the local characteristics of the MRF constrained by the local Markov properties~\cite{koller2009probabilistic} and is convenient to model robotics swarms.

A GRF is a particular application for (\ref{eq:mrf}) when its joint probability density can be represented by the Gibbs measure. A Gibbs measure is a generalization of the canonical ensemble to infinite systems, which gives the probability of the system $\mathbf{X}$ being in the state $x$. Formally, a random field $\mathbf{X}$ is called a GRF if,
\begin{equation}
    P(\mathbf{X} = x) = \frac{1}{Z}e^{-\frac{H(x)}{T}}, \textrm{ with } Z = \sum \limits_{z} e^{-\frac{H(x)}{T}},
    \label{eq:gibbsdistribution}
\end{equation}
where $Z$ is the partition function (normalizing constant); $H(x)$ is a pairwise, nearest-neighbor potential energy; $T$ is interpreted as temperature in the context of statistical physics; and $\frac{1}{Z}e^{-\frac{H(x)}{T}}$ is called Gibbs distribution.  

Researchers in statistical mechanics and mathematics usually applied the GRF to describe the distribution of system configurations at the thermodynamic equilibrium or to measure the probability of such a system to yield the desired state. One of the challenges of directly evaluating~(\ref{eq:gibbsdistribution}) is the high cardinality of the configuration space, which makes the computation of $Z$ intractable.

A typical approach to sequential sampling states in a configuration space given a probability function consists of using Markov Chain Monte Carlo (MCMC) methods, such as the Metropolis algorithm~\cite{hastings1970monte}. A process to parallely sample over~(\ref{eq:gibbsdistribution}) is described in the next section.

%%% end Background %%%



\subsection{Formalization}
\label{subsec:formalization}
Assume a set of $\eta$ homogeneous robots, indexed by $\displaystyle{\mathcal{R} = \{1,...,\eta\}}$, navigating in a bounded region within the two-dimensional Euclidean space\footnote{We assume two-dimensional space for convenience but one can straightforward extend it to three-dimensional space.}. The state of each robot $i$ at time step $t$ is represented by its pose $\mathbf{q}_i ^{(t)}$ and velocity $\dot{\mathbf{q}_i}^{(t)} = \mathbf{v}_i^{(t)}$, which is bounded by $v_{max}$, $||\mathbf{v}_i^{(t)}|| \leq v_{max}$. In addition, robots are driven by a holonomic kinematic model with motion model $\displaystyle{\mathcal{K} : (\mathbf{q}_i^{(t)}, \mathbf{v}_i^{(t)}) \rightarrow (\mathbf{q}_i^{(t+1)})}$. The heterogeneity of the system is modeled by a partition $\tau = \{{\tau}_1, ..., {\tau}_m \}$, with each ${\tau}_k \subset \mathcal{R}$ containing exclusively all robots of type $k$. That is, $\forall (j,k) : j \neq k \ \rightarrow {\tau}_k \cap {\tau}_j = \emptyset$. 

Each robot has a circular sensing range of radius $\lambda$, where it can estimate the relative position and velocity of other robots as well as their type, and also obstacles within the environment. 
%\subsubsection{Obstacles formalization} 
Obstacles are represented as a finite set of points $\displaystyle{\mathcal{O} = \{\mathbf{o}_1, ..., \mathbf{o}_n\}}$. An obstacle detected by robot $i$ consists of a subset of points $\mathcal{O}_i \subset \mathcal{O}$, where $\displaystyle{ \mathbf{o}_j \in \mathcal{O}_i \rightarrow ||\mathbf{o}_j - \mathbf{q}_i|| \leq \lambda}$ and $||\mathbf{o}_j - \mathbf{q}_i||$ is the Euclidean norm between two points. 
%An obstacle detected by the robot $i$ into the sensing range is defined as a finite set of points $\displaystyle{\mathcal{O}_i = \{\mathbf{o}_1, ..., \mathbf{o}_n\}}$, where $\displaystyle{\forall \mathbf{o}_j \in \mathcal{O}_j \rightarrow ||\mathbf{o}_j - \mathbf{q}_i|| \leq \lambda}$.

%\subsubsection{Neighborhood system} 
The neighborhood system for robot $i$, constrained by the sensing range $\lambda$, defines a set of robots: 
%within a circular region of radius equal to the sensing range. That is, the neighborhood system for the robot $i$ is defined as
\begin{equation}
    \mathcal{N}_i \triangleq \{j \in \mathcal{R}: j \neq i, ||\mathbf{q}_j - \mathbf{q}_i|| \leq \lambda \}.
    \label{eq:neighborhood}
\end{equation}
%where $||\mathbf{q}_j - \mathbf{q}_i||$ is the Euclidean distance between robots $i$ and $j$.

\subsection{Extension of the GRF to swarm robotics}
Inspired by the GRF capability in modeling local interactions, here we discuss its concepts in the context of swarm robotics. 
%A similar approach can be seen in the work of Tan et al.~\cite{tan2010decentralized}.
Following the modeling presented in section~\ref{sec:background}, let us define a graph $\mathbf{G} = (\mathcal{R},\mathbf{E})$ with a set of random variables $\mathbf{X} = \{X_i\}_{i \in \mathcal{R}}$, in which each $X_i$ models the random velocity $\mathbf{v}_i$ of robot $i$. A configuration of the system $\mathbf{X}$ is $\displaystyle{\mathbf{x} = \{\mathbf{v}_1,... ,\mathbf{v}_\eta\}}$ where $\mathbf{v}_i \in \Lambda_i$ and represents the velocities performed by each robot.
%A configuration of the system $\mathbf{X}$ is $\mathbf{x} = \{x_{\mathcal{R}_i}, x_{\mathcal{R}_i} \in \Lambda_{\mathcal{R}_i}\}_{\mathcal{R}_i \in \mathcal{R}}$ and represents the velocities performed by each robot.

A neighborhood system on $\mathcal{R}$, given a configuration space $\mathbf{x}$, is a family $\displaystyle{\mathcal{N} = \{\mathcal{N}_{i}\}_{i \in \mathcal{R}}}$, where $\mathcal{N}_i \subset \mathcal{R}$ is the set of neighbors defined in (\ref{eq:neighborhood}) and satisfies $i/\mathcal{N}_i$ and the symmetry $\displaystyle{j \in \mathcal{N}_i \Leftrightarrow i \in \mathcal{N}_j}$. The neighborhood system $\mathcal{N}$ induces the configuration of the graph $\mathbf{G}$ by establishing an edge between each pair $(i,j)$ of robots if and only if $j \in \mathcal{N}_i$.

Until now, our definitions only allow us to calculate the probability of the entire swarm reaching a certain configuration, but what we require here is to sample velocities for each robot given the information about the robots in its neighborhood. Next, we explain how we perform such procedure in a decentralized way using the Gibbs distribution.

\subsection{Parallel Gibbs sampling}
%A remark is that the parallel sampling is possible due to the local nature of the Gibbs potential energy.
Parallel Gibbs sampling implies that all robots are simultaneously updating their velocities based on the configuration $\mathbf{x}$ at time $t$. Such method is possible here due to the local nature of the Gibbs potential energy. %as we present in the following.

Formally, let $t$ denote the temporal index and $\displaystyle{\mathbf{x}^{(t)} = \mathbf{x} = (\mathbf{v}_1, ..., \mathbf{v}_\eta)}$ be the swarm configuration at time $t$. Let $\mathbf{Z}_i(\mathbf{x}) \triangleq \{\mathbf{z}_i : ||\mathbf{z}_i|| \leq v_{max}\}$, where $\mathbf{Z}_i(\mathbf{x}) \subset \Lambda_i$, be the set of possible velocities for robot $i$ given the configuration $\mathbf{x}^{(t)}$.
%For the parallel Gibbs sampling, all robots are simultaneously updating their velocities based on the configuration $\mathbf{x}$ at time $t$. 
Using~(\ref{eq:gibbsdistribution}), robot $i$ updates its velocity $\mathbf{v_i}^{(t)} = \mathbf{v_i}$ to $\mathbf{v_i}^{(t+1)} = \mathbf{\bar v_i}$ with probability
\begin{equation}
    P_i(\mathbf{v_i}, \mathbf{\bar v_i}|\mathbf{x}) = 
    \begin{cases} 
    \frac{e^{-H(\mathbf{\bar v_i}, \mathbf{x}_{\mathcal{R} \setminus i})/T}}{\sum \limits_{\mathbf{z}_j \in \mathbf{Z}_i(x)} e^{-H(\mathbf{z}_j, \mathbf{x}_{\mathcal{R} \setminus i})/T}},& \text{ if } \mathbf{\bar v_i} \in Z_i(\mathbf{x}) \\
    0,& \text{otherwise}.
    \end{cases}
    \label{eq:probglobal}
\end{equation}
Note that (\ref{eq:probglobal}) still depends on the global knowledge at the potential energy $H(\cdot , \mathbf{x}_{\mathcal{R} \setminus i})$. However, if we rewrite~(\ref{eq:potentialenergy2}) as,
\begin{equation}
    \begin{split}
        H(\cdot , \mathbf{x}_{\mathcal{R} \setminus i}) = 
            \left( U_{\{i\}}(\cdot) + \sum \limits_{\forall j \in \mathcal{R} \setminus i} U_{\{j\}}(\mathbf{v}_j) \right) + \\
            \sum \limits_{\forall j \in \mathcal{N}_i}U_{\{i,j\}}(\cdot, \mathbf{v_j}),
    \end{split}
\end{equation}
one may note that the second term inside the parenthesis is constant for $i$, which lets us reduce the form for $H(\mathbf{\bar v_i} , \mathbf{x}_{\mathcal{R} \setminus i})$ and $H(\mathbf{z_i} , \mathbf{x}_{\mathcal{R} \setminus i})$ in~(\ref{eq:probglobal}). This shows the local nature of the Gibbs potential energy and implies that we do not require the knowledge of the entire swarm to sample velocities for a given robot $i$, but only information about its neighbors $\mathcal{N}_i$. Thus, we can rewrite~(\ref{eq:probglobal}) as 
% Due to the local nature of the Gibbs potential energy, we can rewrite~(\ref{eq:potentialenergy2}) for $H(\mathbf{\bar v_i} , \mathbf{x}_{\mathcal{R} \setminus i})$ and $H(\mathbf{z_i} , \mathbf{x}_{\mathcal{R} \setminus i})$ as
% \begin{equation}
%     \begin{split}
%         H(\mathbf{\bar v_i} , \mathbf{x}_{\mathcal{R} \setminus i}) = 
%             \left( U_{\{i\}}(\mathbf{\bar v_i}) + \sum \limits_{\forall j \in \mathcal{R} \setminus i} U_{\{j\}}(\mathbf{v}_j) \right) + \\
%             \sum \limits_{\forall j \in \mathcal{N}_i}U_{\{i,j\}}(\mathbf{\bar v_i}, \mathbf{v_j}),
%     \end{split}
% \end{equation}
% and, 
% \begin{equation}
%     \begin{split}
%     H(\mathbf{z_i} , \mathbf{x}_{\mathcal{R} \setminus i}) = 
%             \left( U_{\{i\}}(\mathbf{z_i}) + \sum \limits_{\forall j \in \mathcal{R} \setminus i} U_{\{j\}}(\mathbf{v}_j) \right) +\\
%             \sum \limits_{\forall j \in \mathcal{N}_i}U_{\{i,j\}}(\mathbf{z_i}, \mathbf{v_j}).
%     \end{split}
% \end{equation}
%Since $H(\mathbf{\bar v_i} , \mathbf{x}_{\mathcal{R} \setminus i})$ and $H(\mathbf{z_i} , \mathbf{x}_{\mathcal{R} \setminus i})$ share a common term (second term inside the parenthesis) constant in $i$, we show that (\ref{eq:probglobal}) does not require the knowledge of the entire swarm to sample velocities for a given robot $i$ and their neighbors $\mathcal{N}_i$. Thus, we can rewrite~(\ref{eq:probglobal}) as
\begin{equation}
    P_i(\mathbf{v_i}, \mathbf{\bar v_i}|\mathbf{x}) = 
    \frac{e^{-\left(U_{\{i\}}(\mathbf{\bar v_i}) + \sum \limits_{\forall j \in \mathcal{N}_i}U_{\{i,j\}}(\mathbf{\bar v_i}, \mathbf{v_j})\right)T^{-1}}}
    {\sum \limits_{\mathbf{z_i} \in \mathbf{Z}_i(x)} e^{-\left(U_{\{i\}}(\mathbf{z_i}) + \sum \limits_{\forall j \in \mathcal{N}_i}U_{\{i,j\}}(\mathbf{z_i}, \mathbf{v_j})\right)T^{-1}}},
    \label{eq:problocal}
\end{equation}
where $\mathbf{\bar v_i} \in \mathbf{Z}_i(\mathbf{x})$.


\subsection{Potential energy}
Here we propose the combination of two potential functions into the potential energy $H(\cdot)$ to achieve simultaneous segregative-flocking behaviors of the swarm.
\subsubsection{Coulomb-Buckingham potential}
The Coulomb-Buckingham potential~\cite{buckingham1938classical} is a combination of the Lennard-Jones potential with the Coulomb potential used to describe the interaction among particles considering their charges. We took advantage of such a mechanism to model the heterogeneity of the swarm by setting the particle charges. The formula for the interaction is
\begin{equation}
\Phi (r)=\varepsilon \left({\frac {6}{\alpha -6}}e^{\alpha} \left(1-{\frac {r}{r_{0}}}\right)-{\frac {\alpha }{\alpha -6}}\left({\frac {r_{0}}{r}}\right)^{6}\right) + \frac {c_{i}c_{j}}{4\pi \varepsilon_0 r},
    \label{eq:cbpotential}
\end{equation}
where $r = ||\mathbf{q}_j - \mathbf{q}_i||$ is the euclidean distance between the particles $i$ and $j$; $\varepsilon$ is the depth of the minimum energy; $r_{0}$ is the minimum energy distance; $\alpha$ is a free dimensionless parameter; $c_i$ and $c_j$ are the charges of the particles $i$ and $j$; and $\varepsilon_0$ is an electric constant. 

We define the interaction among robots $i$ and $j$ by replacing the product $c_i c_j$ by the following function,
\begin{equation}
    C(i,j) = \left(2~\mathbb{1}((i, j) \in \tau_k ) - 1 \right)|c_i c_j|,
\end{equation}
where $\mathbb{1}(\cdot)$ denotes the indicator function. In this way $C(i,j)$ will be positive if robots $i$ and $j$ belong to the same group $\tau_k$ and negative otherwise. Fig.~\ref{fig:cbpotential} illustrates the Coulomb-Buckingham potential.

\begin{figure}[t]
		\centering
		\includegraphics[width=.75\columnwidth]{figures/cbpotential.png}
	\caption{The Coulomb-Buckingham potential function. It depends on the distance $r$ among  robots $i$ and $j$ and a function $C(i,j)$ that produces attractive or repulsive behaviors depending on the heterogeneity among them. %Here we assume $|c_i c_j|= 24$; $\varepsilon = \varepsilon_0 = 0.04$; $r_0 = 1.6$; and $\alpha = 1.0$.
	} 
	\label{fig:cbpotential}
\end{figure}

\begin{figure}[t]
		\centering
		\includegraphics[width=.95\columnwidth]{figures/scheme_transport.pdf}
	\caption{The Coulomb-Buckingham potential function. It depends on the distance $r$ among  robots $i$ and $j$ and a function $C(i,j)$ that produces attractive or repulsive behaviors depending on the heterogeneity among them. %Here we assume $|c_i c_j|= 24$; $\varepsilon = \varepsilon_0 = 0.04$; $r_0 = 1.6$; and $\alpha = 1.0$.
	} 
	\label{fig:occlusion_strategy}
\end{figure}

\subsubsection{Kinetic energy}
We assume classical mechanics to compute the kinetic energy produced by relative velocities of robot $i$ neighbors. Let $\mathbf{V}_i$ define the resultant of the relative velocities among all neighbors within the same partition of the robot $i$. The kinetic energy $\mathbf{E_k}$ relative to robot $i$, is:
\begin{equation}
\mathbf{V}_i = \sum \limits_{\forall j \in \mathcal{N}_i \land (i,j) \in \tau_k} \mathbf{v}_j, \ \ \ \mathbf{E_k}(\mathbf{V}_i) = \frac{1}{2} m (\mathbf{V}_i \cdot \mathbf{V}_i),
\end{equation}
%That is, 
%\begin{equation}
%\mathbf{V}_i = \sum \limits_{\forall j \in \mathcal{N}_i \land (i,j) \in \tau_k} \mathbf{v}_j.  
%\end{equation}
%Thus, the kinetic energy relative to robot $i$, is
%\begin{equation}
%    \mathbf{E_k}(\mathbf{V}_i) = \frac{1}{2} m (\mathbf{V}_i \cdot \mathbf{V}_i)
%\end{equation}
where $m$ is the cumulative mass of the group.




\subsubsection{Combination}
 We combine the Coulomb-Buckingham potential and the kinetic energy to define the potential energy $H(\mathbf{\bar v}_i , \mathbf{x}_{\mathcal{R} \setminus i})$. Here, the individual potential $U_{\{i\}}(\mathbf{\bar v_i})$ represents an obstacle avoidance factor defined by
\begin{equation}
    \begin{split}
            U_{\{i\}}(\mathbf{\bar v_i}) = \sum \limits_{\forall j \in \mathcal{O}_i} \Phi(||\mathcal{K}(\mathbf{q}_i, \bar{\mathbf{v}_i}) - \mathbf{o_j}||),
    \end{split}
    \label{eq:paiwisepot}
\end{equation}
and $\forall j \in \mathcal{O}_i: C(i, j) > 0$.

The nearest-neighbor potential establishes a segregative-flocking factor formulated as
\begin{equation}
    \begin{split}
            \sum \limits_{\forall j \in \mathcal{N}_i}U_{\{i,j\}}(\mathbf{\bar v_i}, \mathbf{v_j}) = 
            \sum \limits_{\forall j \in \mathcal{N}_i} \Phi(||\mathcal{K}(\mathbf{q}_i, \bar{\mathbf{v}_i}) - \mathcal{K}(\mathbf{q}_j, {\mathbf{v}_j})||) + \\
            \mathbf{E_k}(\mathbf{V}_i) + \mathbf{E_k}(v_{max} - \bar{\mathbf{v}_i}),
    \end{split}
    \label{eq:nearestneighborpot}
\end{equation}
where the first term defines the attraction and repulsion among two robots and the second one is the relative velocity of the neighbors. Since we compute the kinetic energy using relative velocities, when $\mathbf{E_k}(\mathbf{V}_i) \rightarrow 0$, there is a duality on the behavior produced by the robots. More specifically, one may not differentiate if the robots are stationary or moving with the same velocities. To avoid such duality, we added a third term to force the robot $i$ to reach its maximum speed.

\subsection{Sampling algorithm}
Finally, given the probability function~(\ref{eq:problocal}) and the potential energy defined by combination of (\ref{eq:paiwisepot}) and~(\ref{eq:nearestneighborpot}) one may use a MCMC algorithm to sample velocities for a given robot $i$. In this work, we use the Metropolis-Hastings algorithm~\cite{peskun1973optimum} for sampling the velocities.
presented in  Algorithm~\ref{alg:metropolis}.

%algorimo retirado e colocado no temp.tex
\begin{algorithm}[t]
\caption{Calculate robot $i$ velocity at time $t+1$}\label{alg:metropolis}
\Procedure{Update}{$\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)}$} 
 \State $\mathbf{V}^{(0)} \gets \mathbf{v_i}^{(t)}$, \Comment{Set of velocities} 
 \State $\mathbf{U}^{(0)} \gets H(\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)})$, \Comment{Set of potential energies} 
 \For{$k \gets 1$ to $\mathcal{I}$}
%  \State $\mathbf{v}_{prev} \gets \mathbf{V}$(end),  \Comment{Get the last element of $\mathbf{V}$} 
%  \State $\mathbf{u}_{prev} \gets \mathbf{U}$(end),  \Comment{Get the last element of $\mathbf{U}$} 
 \State $\bar{\mathbf{v}} \gets N(\mathbf{v_i}^{(t)}, \mathbf{\Sigma})$,    \Comment{Gaussian sampling} 
 \State $\bar{\mathbf{u}} \gets  H(\mathbf{q_i}^{(t)}, \bar{\mathbf{v}})$,
 \State $\Delta E \gets \bar{\mathbf{u}} - \mathbf{U}^{(k-1)}$,      \Comment{Potential energy variation}
 \State $g \gets exp(-\Delta E)$,   \Comment{Compute the gibbs energy}
 \State $r \gets \mathcal{U}(0, 1)$,   \Comment{Uniform sampling}
 \If{$(\Delta E < 0) \lor (r < g)$ } \Comment{Sample is accepted}
    \State $\mathbf{V}^{(k)} \gets \bar{\mathbf{v}}$,
    \State $\mathbf{U}^{(k)} \gets \bar{\mathbf{u}}$,
    \Else \Comment{Sample is rejected}
    \State $\mathbf{V}^{(k)} \gets  {\mathbf{V}^{(k-1)}}$,
    \State $\mathbf{U}^{(k)} \gets  {\mathbf{U}^{(k-1)}}$,
    \EndIf
 \EndFor
%  \State $\mathbf{V} \gets \mathbf{V}^{(j,...,\mathcal{I})}$, \Comment{Reject the first j velocities}
 \State $\mathbf{v_i}^{(t+1)} \gets  (\mathbf{V}^q + ...+\mathbf{V}^\mathcal{I})/(\mathcal{I}-q)$, \Comment{Average velocity}
 \State \textbf{return} $\mathbf{v_i}^{(t+1)}$
\EndProcedure
\end{algorithm}

==> sections/temp/SavedText.tex <==
% Introduction

Swarm robotics is a field of robotics that takes inspiration from emergent behaviors, commonly observed in natural systems, to design decentralized control methods in a scalable fashion relying only on local sensing and communication capabilities. 
Due to the scalability factor, swarm robotics is suitable to automate tasks that are beyond the capacity of single robot systems. Besides, it is potentially more cost-effective and resilient to different types of failures, ranging from hardware to software~\cite{parker2006collective}. 
%; when one robot fails or makes a mistake, the others can still complete the task successfully

Due to the progressive advancement in technology that has enabled the mass production of increasingly smaller robots~\cite{miskin2020electronically}, researchers are light on decentralized control methods that produce desired collective behaviors of a large number of robots~\cite{schranz2020swarm}. Several real-world applications can benefit from using control methods based on swarm behaviors, such as area coverage, surveillance, reconnaissance, transport, foraging, among others~\cite{tarapore2020sparse, tan2013research}.

In particular, swarm robots capable of cooperatively transporting objects may be suitable for many applications with high economic and societal impact potential. For instance, one may use swarm robots to waste retrieval and disposal, demining, or operations requiring object manipulation in environments where direct human intervention is impossible or impractical~\cite{alkilabi2017cooperative}.%, such as in space or the deep sea~\cite{alkilabi2017cooperative}.




==> sections/temp/temp.tex <==
\subsection{Applications} % or Other behaviors
As we state,  the combination of segregative and flocking behaviors allows the execution of several complex tasks. Further, we intend to deal with such tasks using the methodology presented in this work. For instance, we aim to investigate swarm transportation and shape-formation in the context of heterogeneity groups. Fig.~\ref{fig:segregationexp} shows an initial step toward to shape-formation. 

\begin{figure}[h]
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0001.png}
		\caption{$n=0$}
		\label{fig:rangerobots}
	\end{subfigure}%
    \hspace*{-1.2em}
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0042.png}
		\caption{$n=200$}
		\label{fig:rangegroups}
	\end{subfigure}%
    \hspace*{-1.2em}
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0322.png}
		\caption{$n=1600$}
		\label{fig:shapeformation}
	\end{subfigure}%
	\caption{Initial steps toward shape-formation task. Virtual points with heterogeneous attraction are placed in the environment so that robots of a specific type are attracted, resulting in the formation of structures. A video is available at \url{https://youtu.be/uJs0fwiQHIc}.} % footnote
	\label{fig:segregationexp}
\end{figure}







==> sections/temp/tesis.tex <==
\begin{table*}[!h]
\caption{Main characteristics of research works using pushing-only transport strategy.}
\label{tab:comparision}
\resizebox{\textwidth}{!}{\begin{tabular}{lllllllllllllll}
\toprule
\multicolumn{1}{c}{\textbf{Studies}} & \multicolumn{1}{c}{\textbf{Control method}} & & \multicolumn{4}{c}{\textbf{Experimental setup}} & & \multicolumn{1}{c}{\textbf{Scalability}} & \multicolumn{2}{c}{\textbf{Adaptability test}} & & \multicolumn{3}{c}{\textbf{Robustness test}} \\ \cmidrule{4-7} \cmidrule{10-11} \cmidrule{13-15} 
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\end{tabular}}} & &
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ robots\end{tabular}}} & 
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Env. with \\ obstacles\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Transport \\ direction\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Random initial \\ position\end{tabular}}} & &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\end{tabular}}} & 
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Robot\\ failure \end{tabular}}} & 
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Change in the\\ environment\end{tabular}}} & &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Object\\ mass\end{tabular}}} & 
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Object\\ shape\end{tabular}}} &
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Object\\ size\end{tabular}}} \\ \midrule
Kube and Bonabeau, 2000~\cite{kube2000cooperative} & behavior-based  & & 2-20  & no & towards a goal & no & & strong & no & no & & no & no & yes\\
Yamada and Saito, 2001~\cite{yamada2001adaptive} & behavior-based  & & 4  & no & towards a goal & no & & weak & yes & yes & & no & no & no\\
Fujisawa et al., 2013~\cite{fujisawa2013cooperative} & behavior-based  & & 4-10  & no & towards a goal & yes & & strong & yes & yes & & yes & no & no\\
Jianing Chen et al., 2015~\cite{chen2015occlusion} & behavior-based  & & 20  & yes & towards a goal & yes & & strong & no & no & & yes & yes & yes\\
Alkilabi et al., 2018~\cite{alkilabi2018evolving} & automatic  & & 2-6  & no & towards a goal & no & & strong & no & no & & yes & no & yes\\
\textbf{Ours} & \textbf{other} & & \textbf{6-40}  & \textbf{yes} & \textbf{towards a goal} & \textbf{yes} & & \textbf{strong} & \textbf{yes} & \textbf{yes} & & \textbf{yes} & \textbf{yes} & \textbf{yes} \\ 
\bottomrule
\end{tabular}}
\end{table*}

\section{Related Work}
\label{sec:relatedwork}
Over the years, a wide range of control  and coordination methods have been proposed to perform cooperative object transport using multiple robots.
Recently, Tuci et al.~\cite{tuci2018cooperative} presented a review of the state-of-the-art works in cooperative transport which categorizes the most common strategies used for transportation into three types: pushing, caging and grasping.

Pushing strategies consider that the robots are not attached to the object. They provide a simple way of manipulating relatively large objects and do not require any sophisticated mechanism to apply forces to the object. Pushing is also interesting because, unlike other strategies, it allows robots to aggregate and apply forces to specific points on the object, enabling the transport large and heavy objects when the number of robots is increased.

Caging can be considered a special case of the pushing. It requires the robots to coordinate and distributed themselves along the object to enclosure it and maintain their formation during transport. This strategy is particularly interesting because it allows fast maneuvers with the object, being more stable than pushing, without depending on complex mechanisms for transportation. However, it normally demands a specific number of robots which imposes a limit on the mass of the object to be transported. Also, it may become more complex depending on the shape of the object, requiring some information about it.

The grasping strategy requires robots that are able to physically attach to the object and apply either pushing or pulling forces in order to transport it. This strategy allows higher dexterity during the transport of objects. However, similar to the caging strategy, it is also restricted to a specific number of robots, imposing a limit on the load capacity. Also, it may not be always suitable for swarm robots depending of the complexity of the physical mechanisms.

The strategy used in this work consists of push the object towards its goal location. We use such strategy because it allows the use of less sophisticated robots, providing a more realistic scenario for systems with a large number of robots. We also assume that the robot does not rely on direct communication system. Although in principle the communication among robots should improve their ability to cooperate, as a system grows in number, non-communicating systems should scale more easily.

Next, we review the main works of literature that use the pushing strategy and compare the most related approaches with ours. Besides, given the reasonable amount of work in the literature, we also restrict our comparison to only those approaches that use indirect communication (see Tuci et al.~\cite{tuci2018cooperative}, for more details about the other works). Table~\ref{tab:comparision} summarizes the main characteristics of each approach, and in the following, we review and compare these works with ours, by emphasizing robustness, scalability and adaptability.


Kube et al.~\cite{kube1993collective} presented one of the first studies that formally dealt with the dynamics of cooperative transport. The authors demonstrate that coordinated efforts, produced by a homogeneous group of simple robots pushing an object, are possible without the use of a direct communication mechanism. To demonstrate this hypothesis, they presented two strategies: the first one was a subsumption-style behavior-based controller with a fixed priority behavior arbitration; and the second one using reflexive behaviors and adaptive logic networks, trained with a supervised training algorithm, for behavior arbitration. Further, in Kube and Zhang~\cite{kube1997task}, the authors extend the original work by constructing a new robot for experimentation. In Kube and Bonabeau~\cite{kube2000cooperative}, they proposed the addition of a stagnation recovery strategy avoiding deadlock conditions in which the robots cancel the pushing forces on the object depending on where they are positioned around the object. Also, they extend their approach to allow the robot to push the object towards a fixed goal position, and, performed experiments to test the robustness and scalability of their method.
%of their method against the size of a box object and scalability of the system.


Yamada and Saito~\cite{yamada2001adaptive} also presented theoretical and experimental foundations to support the assumption that robots can transport objects without using direct communication. Unlike previous works, the authors demonstrated that the use of indirect communication also allows the transport of an object towards a goal location considering a dynamic environment. %Their approach consists of using an action selection method to design a behavior-based control method that, despite the cooperative transport, also allows the swarm to be adaptive to a dynamic environment in which the number of robots and the mass of the object difficulty change. 
Their approach consists of using an action selection method to design a behavior-based control method that is robust to a small change in the environment, such as increase the number of robots or the mass of the object. 
To evaluate the performance of their approach, the authors performed full real experiments using four robots showing that the robots can operate in a simple environment where individual robots are required to push a light object, or in complex environments where multiple robots are required to cooperatively push a heavy object. Although their approach allows adaptability to small changes in the environment, the authors did not evaluate the robustness of the method to objects of different shapes, masses, and sizes. Furthermore, the method does not seem to scale easily as the system grows in number. 


Fujisawa et al., 2013~\cite{fujisawa2013cooperative} presented a cooperative transport approach that uses an interesting mechanism for indirect communication via artificial pheromones as seen in ants. Basically, such mechanism allows the robots to sense and lay on the terrain a volatile alcohol substance mimicking the effect of pheromone during trail formation. The authors also proposed a behavior-based algorithm using a deterministic finite automaton, which allows the robots to perform a random search to find a food item (i.e., a heavy object), and to transport it to a goal location (i.e., the nest). To evaluate the efficiency of the proposed system, the authors perform experiments with up to 10 robots demonstrating the adaptability and robustness of their approach. They showed that the system remains stable when the weight of the object is changed and when considered failures in some robots, incapacitating them from carrying out the task. With respect to experiments that assess the impact of using the pheromone-based communication mechanism, they show that such a mechanism is effective only with a relatively small number of robots in the environment. For a larger group of robots, they observed an irrelevant impact on the completion time, as many robots are likely to find the food and begin the cooperative transport before the trail is formed. Although the authors present experiments that evaluated the adaptability and robustness of the proposed method, the work does not assess the scalability of the system and also the robustness of the method as to the shape and size of the object changes.


Jianing Chen et al.~\cite{chen2015occlusion} proposed another behavior-based strategy for cooperative transport that, instead of trying to deal with the occlusion caused by the object when the robots detect the goal location, they take the advantage that if the robots push the object while not detecting the goal, it implies moving the object approximately towards it. This simple behavior results in transporting the object towards the goal without using any form of direct communication. To evaluate their strategy, they perform experiments using a group of twenty robots to transport objects of different shapes towards their goals. They also provide an analytical proof of the effectiveness of the method, and results of successful empirical tests are discussed. In addition, the authors also demonstrated other interesting experiments in which they consider the goal location as a mobile robot remotely controlled by a human, showing potential applications in the context of human-robot interaction. The work was further extended with this focus in Kapellmann-Zafra et al.~\cite{kapellmann2016using}. Although the authors demonstrated the scalability and robustness of the system to different types of objects, tests evaluating the adaptability of the system to failures or changes in the environment were not performed.


Differently from previous approaches, Alkilabi et al.~\cite{alkilabi2017cooperative} proposed the use of an automatic control method to demonstrate that effective coordination of forces to transport heavy objects to an arbitrary direction can be obtained by a group of robots equipped with a minimalist sensory apparatus, and with no means of direct communication, allowing the robots to only perceive the movements of the object. The robot controller is composed by a continuous time recurrent neural network and evolutionary algorithm is employed to set its parameters. The best instance evolved of the controller was extensively tested on physical robots to transport objects of different sizes and masses to an arbitrary direction. Further, Alkilabi et al.~\cite{alkilabi2018evolving} presented a complementary study extending their neural-controller with mechanisms to direct the transport towards a specific target location. The authors show that the transport strategies are scalable with respect to the group size, and robust enough to deal with boxes of various mass and size. Despite this work presenting an interesting solution and performed an satisfactory set of experiments, the strategy still requires that robots start with a direct view of the object, and also does not consider objects with different shapes or obstacles in the environment.

In general, as we investigate and compare works that assume less sophisticated robots (i.e., uses indirect communication and a push-only strategy), we note an interesting trend. All the previous studies, under the mentioned restrictions, assume homogeneous robots and, still, do not exploit possible advantage of heterogeneity. As it seems to be a common census to produce methods that move the object to a certain location, we imagine that one may take advantage of heterogeneity to assist in the navigation of the object through the environment. % mais observacoes

This paper extends a preliminary study described in Rezeck et al.~\cite{arxivGIBBS} to allows a swarm of robots to coordinated their motion to cohesive navigate through a bounded environment and cooperatively transport an object toward its goal location.
Unlike the approaches presented earlier, our control method is not based on pre-synthesized behaviors or automatic learning methods, but on the modeling of the swarm as a dynamic Gibbs Random Fields (GRF). The swarm behavior emerges through the use of appropriate potential functions, and the control of the robot, that allows the robots to produce the desired behavior, results from the use of Markov Chain Monte Carlo (MCMC) method. Although our approach is different from others in the literature, since it implicitly emerges two swarming behaviors, our method provides scalability, adaptability and robustness to several factors (discussed further). 


%Moreover, although our approach produces flocking behaviors, we do not use or extend the mechanism proposed by Reynolds~\cite{reynolds1987flocks}. We model the swarm using dynamic Gibbs Random Fields (GRF), which provide a robust framework for dealing with spatial correlated probabilities. We have been inspired by Tan et al.~\cite{tan2010decentralized} that used GRF to self-organize homogeneous robots. Besides the use of heterogeneous robots, there are other crucial differences between our work and~\cite{tan2010decentralized}: we model a continuous movement of the robots in a bounded environment and limit the robots' maximum velocities, while Tan et al. consider a discrete and a bounded environment and assume lattices as their environment. In addition, we introduce a different potential function that makes all the difference in our approach. In contrast with previous work, we adopt a Coulomb-Buckingham Potential~\cite{buckingham1938classical} coupled with a Kinetic Energy term to model the robots' interactions.



